Event-Keyed Summarization

We introduce event-keyed summarization (EKS), a novel task that marries traditional summarization and document-level event extraction, with the goal of generating a contextualized summary for a specific event, given a document and an extracted event structure. We introduce a dataset for this task, MUCSUM, consisting of summaries of all events in the classic MUC-4 dataset, along with a set of baselines that comprises both pretrained LM standards in the summarization literature, as well as larger frontier models. We show that ablations that reduce EKS to traditional summarization or structure-to-text yield inferior summaries of target events and that MUCSUM is a robust benchmark for this task. Lastly, we conduct a human evaluation of both reference and model summaries, and provide some detailed analysis of the results.

==> appendices/additional_results.tex <==
% \begin{table}[]
%     \centering
%     \adjustbox{max width = \columnwidth}{
%     \begin{tabular}{ll|cccccc}
%     \toprule
%     & & Gold$\rightarrow$Gen & Gold$\leftarrow$Gen & Average & Doc$\rightarrow$Gen & Doc$\rightarrow$Gen & Doc$\rightarrow$Gold\\
%     \midrule
%     & temp + doc & 39.9 & 30.6 & 35.2 & 37.4 & 37.4 & 41.2\\
%     $\textsc{BART}$ & temp only & 15.4 & 8.8 & 12.1 & 12.2 & 12.2 & 41.2\\
%     & doc only & 18.3 & 11.8 & 15.1 & 41.0 & 41.0 & 41.2\\
%     \midrule
%     & temp + doc & 36.8 & 28.5 & 32.6 & 40.6 & 40.6 & 41.2\\
%     $\textsc{PEGASUS}$ & temp only & 30.6 & 7.9 & 19.3 & 19.8 & 19.8 & 41.2\\
%     & doc only & 18.8 & 13.0 & 15.9 & 42.2 & 42.2 & 41.2\\
%     \midrule
%     & temp + doc & 43.1 & 30.5 & 36.8 & 40.6 & 40.6 & 41.2\\
%     $\textsc{T5}$ & temp only & 27.4 & 7.6 & 17.5 & 16.5 & 16.5 & 41.2\\
%     & doc only & 18.2 & 12.5 & 15.3 & 42.4 & 42.4 & 41.2\\
%     \midrule
%     & temp + doc & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & -\\ % 770M 
%     $\textsc{Llama7B}$ & temp only & - & - & - & - & -\\
%     & doc only & - & - & - & - & -\\
%     \midrule
%     & temp + doc & 30.6 & 43.0 & 36.8 & 40.8 & 40.8 & 41.2\\
%     $\textsc{ChatGPT}$ & temp only & - & - & - & - & -\\
%     & doc only & - & - & - & - & -\\
%     \midrule
%     & temp + doc & 45.0 & 40.3 & 42.7 & 38.8 & 38.8 & 41.2\\
%     $\textsc{GPT4}$ & temp only & - & - & - & - & -\\
%     & doc only & - & - & - & - & -\\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{NLI Evaluation for the models}
%     \label{tab:nli_eval}
% \end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{l|ccc}
%     \toprule
%          & \textbf{P} & \textbf{R} & $\textbf{F}_1$ \\
%     \midrule
%         BART & 78.6 & 66.0 & 71.8 \\
%         PEGASUS & 74.0 & 62.3 & 67.6 \\
%         T5 & 80.6 & 63.3 & 70.9 \\
%         ChatGPT & 57.7 & 62.9 & 60.2 \\
%         GPT-4 & 70.2 & 65.2 & 67.6 \\
%     \bottomrule
%     \end{tabular}
%     \caption{CEAF-REE scores for temp+doc models, averaged over three runs/prompts}
%     \label{tab:ceaf_ree_scores}
% \end{table}




==> appendices/temp-lit-review.tex <==
\subsection{Information Extraction based Summarization}
\paragraph{\cite{s-hussain-etal-2022-event}} some stuff


\paragraph{\cite{}}


\subsection{Controlled Summarization}
\paragraph{\cite{fan-etal-2018-controllable}} Summaries to follow user preferences. 

\paragraph{\cite{he-etal-2022-ctrlsum}} Summaries for user preferences, also event-centric



\subsection{Evaluating Eval Metrics}
\paragraph{\cite{deutsch-etal-2021-statistical}} An evaluation of evaluation metrics shows high uncertainty in the reliability of automatic metrics. 

\paragraph{\cite{fabbri-etal-2021-summeval}}


\paragraph{Looking for a Few Good Metrics: Automatic Summarization Evaluation - How Many Samples Are Enough?} evaluating against multiple references results in higher correlation scores with human judgments. however, a single-reference setting is sufficient for the metric to be effective


\paragraph{\cite{rankel-etal-2013-decade}} variants of the ROUGE metric using TAC datasets.


\paragraph{\cite{graham-2015-evaluating}} different ROUGE metric variants and compared it against the BLEU metric on the DUC datasets.

\paragraph{\cite{maynez-etal-2020-faithfulness}} "However, our analysis does show that pretrained models are better summarizers not only in terms of raw metrics, i.e., ROUGE, but also in generating faithful and factual summaries as evaluated by humans. Furthermore, we show that textual entailment measures better correlate with faithfulness than standard metrics, potentially leading the way to automatic evaluation metrics as well as training and decoding criteria.
